Ties Matter: Meta-Evaluating Modern Metrics with Pairwise Accuracy and Tie Calibration

Kendall's tau is frequently used to meta-evaluate how well machine translation (MT) evaluation metrics score individual translations. Its focus on pairwise score comparisons is intuitive but raises the question of how ties should be handled, a gray area that has motivated different variants in the literature. We demonstrate that, in settings like modern MT meta-evaluation, existing variants have weaknesses arising from their handling of ties, and in some situations can even be gamed. We propose instead to meta-evaluate metrics with a version of pairwise accuracy that gives metrics credit for correctly predicting ties, in combination with a tie calibration procedure that automatically introduces ties into metric scores, enabling fair comparison between metrics that do and do not predict ties. We argue and provide experimental evidence that these modifications lead to fairer ranking-based assessments of metric performance.

==> figures/dataset_sizes.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccc}
        \toprule
        \bf LP & \bf \#Systems & \bf \#Segments \\
        \midrule
        en$\rightarrow$de & 13 & 1315 \\
        zh$\rightarrow$en & 14 & 1875 \\
        en$\rightarrow$ru & 15 & 1315 \\
        \bottomrule
    \end{tabular}
    \caption{The number of systems and segments per system rated with MQM scores in the WMT'22 metrics shared task.}
    \label{tab:dataset_sizes}
\end{table}


==> figures/unbabel_ties.tex <==
\begin{table}[hbt!]
    \centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{\bf \#Pairs} & \multicolumn{2}{c}{\bf Google} & & \multicolumn{2}{c}{\bf Unbabel} \\
        \cmidrule{2-3} \cmidrule{5-6}
        & \bf \#Ties & \bf \#Zero-Ties & & \bf \#Ties & \bf \#Zero-Ties \\
        \midrule
        138k & 61k (44\%) & 40k (29\%) & & 51k (37\%) & 40k (29\%) \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The number of ties in the group-by-item correlations using either the Google or Unbabel normalization methods for WMT'22 en-ru.}
    \label{tab:unbabel_ties}
\end{table}

==> figures/unique_scores.tex <==
\begin{table}[]
    \centering
    \begin{adjustbox}{width=\columnwidth}
\begin{tabular}{lrrr}
\toprule
                            \bf Metric &  \bf en-de & \bf   zh-en & \bf   en-ru \\
\midrule
                     COMET-22 &  28942 &  35433 &  31409 \\
                      COMET-QE &  29312 &  35519 &  31407 \\
                     COMETKiwi &  28942 &  35417 &  31307 \\
                GEMBA-Dav3-DA &     16 &     14 &     14 \\
             HWTSC-Teacher-Sim &  22602 &  31719 &  24419 \\
                     MaTESe-QE &     15 &     26 &     11 \\
                       MaTESe &     18 &     26 &     15 \\
                         MEE4 &  19981 &  30357 &  22348 \\
         MetricX\_XXL\_MQM\_2020 &  28063 &  35011 &  30646 \\
                  MS-COMET-22 &  28181 &  35368 &  31369 \\
                MS-COMET-QE-22 &  28735 &  35210 &  31242 \\
                         REUSE &  20090 &  30491 &  22209 \\
                      SEScore &  29321 &  35549 &      - \\
                    UniTE-ref &  20761 &  30557 &  25267 \\
                     UniTE-src &  20762 &  30560 &  23175 \\
\bottomrule
\end{tabular}
\end{adjustbox}
    \caption{The number of unique scores output by the WMT'22 metric submissions and GEMBA.
    GEMBA and \matese are notably outliers and effectively act as classifiers instead of regression models.}
    \label{tab:unique_scores}
\end{table}
